Explaining Chemical Toxicity using Missing Features

Chemical toxicity prediction using machine learning is important in drug development to reduce repeated animal and human testing, thus saving cost and time. It is highly recommended that the predictions of computational toxicology models are mechanistically explainable. Current state of the art machine learning classifiers are based on deep neural networks, which tend to be complex and harder to interpret. In this paper, we apply a recently developed method named contrastive explanations method (CEM) to explain why a chemical or molecule is predicted to be toxic or not. In contrast to popular methods that provide explanations based on what features are present in the molecule, the CEM provides additional explanation on what features are missing from the molecule that is crucial for the prediction, known as the pertinent negative. The CEM does this by optimizing for the minimum perturbation to the model using a projected fast iterative shrinkage-thresholding algorithm (FISTA). We verified that the explanation from CEM matches known toxicophores and findings from other work.

==> CEM for Molecule Toxicity - Extended Abstract/tbl_SA.tex <==
\begin{table}[t]
    \begin{center}
    \vspace{-0.1in}
    \caption{
        Structural alerts identified by the CEM match known general toxicophores (see \citealp{Kazius2005}).
    }%
    \label{tbl:tox_SA}
    \scalebox{0.85}{
        \begin{tabular}{ccccc}
            \toprule
            {General}
            & \multicolumn{2}{c}{~~~~~~Pertinent Negative}
            & \multicolumn{2}{c}{Pertinent Positive}
            \\
            {Toxicophore} & {SA} & {Eg} & {SA} & {Eg} 
            \\
            \midrule 
            % Phenolic OH
            \multirow{2}{*}{Phenolic OH} & 
            {\footnotesize -cc(O)c-} & (1) & 
            \multirow{2}{*}{\footnotesize -cO} & \multirow{2}{*}{(3)}
            \\
            & {\footnotesize -cO} & (1, 2) & &
            \\
            \hline
            % Aliphatic halides
            \multirow{1}{*}{Aliphatic halides} & 
            {\footnotesize Br} & (1, 2) & 
            {\scriptsize -cc(c(F)(F)F)cc-} & (3)
            \\
            (Cl, Br, I, F) & {\footnotesize Br} & (2) & 
            {\footnotesize -c(Cl)} & (4)
            \\
            \hline
            % Polycyclic aromatic system 
            \multirow{1}{*}{Polycyclic} & 
            \multirow{2}{*}{\footnotesize -c(ccc(c)c)c-} \hspace{-2mm} & \multirow{2}{*}{(1)} & & 
            \\
            aromatic system 
            \\
            \hline
            % Aromatic nitro
            \multirow{1}{*}{Aromatic nitro} & 
            {\scriptsize -ccc(N\pion(O\nion)=O)c(N\pion)c-} \hspace{-4mm} & (1) & 
            {\scriptsize N, O\nion, N\pion=O} \hspace{-2mm} & (3) 
            \\
            \bottomrule
        \end{tabular}
    }
    \end{center}
    \vspace{-0.25in}
\end{table}

==> CEM for Molecule Toxicity - Extended Abstract/tbl_tox_MT-DNN.tex <==
\begin{table}[h!]
    \begin{center}
    \caption{
        Performance on toxicity prediction using MT-DNN for all 12 Tox21 tasks and ClinTox task (CT-TOX). The reported metrics are ROC AUC, accuracy, balanced accuracy, true negative rate, true positive rate, precision, recall, and the F1 score. Refer to Table~\ref{tbl:tox_RF} for a comparison with random forest, the MT-DNN achieves much better true positive, recall and F1 score with slight penalty on AUC.
    }%
    \label{tbl:tox_prediction} 
    \scalebox{0.85}{
        \begin{tabular}{r|
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        }
            \toprule
            {Task}
            & {AUC}
            & {ACC}
            & {BAC}
            & {TN}
            & {TP}
            & {PR}
            & {RC}
            & {F1}
            \\
            \midrule
            % \underline{Train} & & & & \\[0.5mm]
            NR-AR & 0.72 & 0.97 & 0.73 & 0.99 & 0.46 & 0.98 & 0.46 & 0.55  \\
            NR-Aromatase & 0.78 & 0.95 & 0.65 & 0.99 & 0.31 & 0.96 & 0.31 & 0.41  \\
            NR-PPAR-$\gamma$ & 0.75 & 0.97 & 0.61 & 0.99 & 0.23 & 0.96 & 0.23 & 0.31  \\
            SR-HSE & 0.75 & 0.94 & 0.61 & 0.99 & 0.23 & 0.94 & 0.23 & 0.32  \\
            NR-AR-LBD & 0.82 & 0.98 & 0.78 & 0.99 & 0.56 & 0.99 & 0.56 & 0.66  \\
            NR-ER & 0.69 & 0.88 & 0.64 & 0.96 & 0.32 & 0.89 & 0.32 & 0.40  \\
            SR-ARE & 0.78 & 0.86 & 0.67 & 0.95 & 0.39 & 0.88 & 0.39 & 0.47  \\
            SR-MMP & 0.87 & 0.89 & 0.75 & 0.96 & 0.54 & 0.93 & 0.54 & 0.62  \\
            NR-AhR & 0.85 & 0.91 & 0.73 & 0.96 & 0.50 & 0.93 & 0.50 & 0.55  \\
            NR-ER-LBD & 0.78 & 0.96 & 0.69 & 0.99 & 0.38 & 0.97 & 0.38 & 0.48  \\
            SR-ATAD5 & 0.75 & 0.96 & 0.61 & 0.99 & 0.22 & 0.97 & 0.22 & 0.32  \\
            SR-p53 & 0.79 & 0.94 & 0.64 & 0.99 & 0.29 & 0.96 & 0.29 & 0.40 \\
            CT-TOX & 0.79 & 0.92 & 0.61 & 0.97 & 0.25 & 0.84 & 0.25 & 0.31 \\[1pt]
            \hdashline
            \rule{0pt}{0.8\normalbaselineskip}  % <- create a tiny gap
            Average	& 0.78 & 0.93 & \textbf{0.67} & 0.98 & \textbf{0.36} & 0.94 & \textbf{0.36} & \textbf{0.45} \\
            \bottomrule
        \end{tabular}
    }
    \end{center}
    % \vspace{-0.2in}
\end{table}

==> CEM for Molecule Toxicity - Extended Abstract/tbl_tox_RF.tex <==
\begin{table}[!h]
    \begin{center}
    \caption{
        Performance on toxicity prediction for Random Forest on all 12 Tox21 tasks and ClinTox task (CT-TOX). The reported metrics are ROC AUC, accuracy, balanced accuracy, true negative rate, true positive rate, precision, recall, and the F1 score.
    }%
    \label{tbl:tox_RF} 
    \scalebox{0.85}{
        \begin{tabular}{r|
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        }
            \toprule
            {Task}
            & {AUC}
            & {ACC}
            & {BAC}
            & {TN}
            & {TP}
            & {PR}
            & {RC}
            & {F1}
            \\
            \midrule 
            % \underline{Train} & & & & \\[0.5mm]
            NR-AR & 0.78 & 0.98 & 0.73 & 0.99 & 0.46 & 0.99 & 0.46 & 0.60 \\
            NR-Aromatase & 0.81 & 0.96 & 0.60 & 0.99 & 0.21 & 0.98 & 0.21 & 0.32 \\
            NR-PPAR-gamma & 0.82 & 0.97 & 0.56 & 0.99 & 0.12 & 0.99 & 0.12 & 0.20 \\
            SR-HSE & 0.77 & 0.95 & 0.56 & 0.99 & 0.13 & 0.97 & 0.13 & 0.22 \\
            NR-AR-LBD & 0.85 & 0.98 & 0.77 & 0.99 & 0.54 & 0.99 & 0.54 & 0.66 \\
            NR-ER & 0.72 & 0.89 & 0.60 & 0.98 & 0.21 & 0.93 & 0.21 & 0.32 \\
            SR-ARE & 0.81 & 0.86 & 0.61 & 0.99 & 0.24 & 0.94 & 0.24 & 0.36 \\
            SR-MMP & 0.88 & 0.89 & 0.67 & 0.98 & 0.36 & 0.95 & 0.36 & 0.49 \\
            NR-AhR & 0.89 & 0.91 & 0.65 & 0.99 & 0.32 & 0.96 & 0.32 & 0.45 \\
            NR-ER-LBD & 0.80 & 0.96 & 0.65 & 0.99 & 0.31 & 0.99 & 0.31 & 0.45 \\
            SR-ATAD5 & 0.84 & 0.96 & 0.55 & 0.99 & 0.10 & 0.97 & 0.10 & 0.18 \\
            SR-p53 & 0.83 & 0.95 & 0.56 & 0.99 & 0.13 & 0.99 & 0.13 & 0.22 \\
            CT-TOX & 0.76 & 0.92 & 0.55 & 0.98 & 0.13 & 0.85 & 0.13 & 0.19 \\[1pt]
            \hdashline
            \rule{0pt}{0.8\normalbaselineskip}  % <- create a tiny gap
            Average & \textbf{0.81} & 0.94 & 0.62 & 0.99 & 0.25 & 0.96 & 0.25 & 0.36 \\
            \bottomrule
        \end{tabular}
    }
    \end{center}
    % \vspace{-0.2in}
\end{table}

==> tbl_tox_MT-DNN.tex <==
\begin{table}[h!]
    \begin{center}
    \caption{
        Performance on toxicity prediction using MT-DNN for all 12 Tox21 tasks and ClinTox task (CT-TOX). The reported metrics are ROC AUC, accuracy, balanced accuracy, true negative rate, true positive rate, precision, recall, and the F1 score. Refer to Table~\ref{tbl:tox_RF} for a comparison with random forest, the MT-DNN achieves much better true positive, recall and F1 score with slight penalty on AUC.
    }%
    \label{tbl:tox_prediction} 
    \scalebox{0.85}{
        \begin{tabular}{r|
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        }
            \toprule
            {Task}
            & {AUC}
            & {ACC}
            & {BAC}
            & {TN}
            & {TP}
            & {PR}
            & {RC}
            & {F1}
            \\
            \midrule
            % \underline{Train} & & & & \\[0.5mm]
            NR-AR & 0.72 & 0.97 & 0.73 & 0.99 & 0.46 & 0.98 & 0.46 & 0.55  \\
            NR-Aromatase & 0.78 & 0.95 & 0.65 & 0.99 & 0.31 & 0.96 & 0.31 & 0.41  \\
            NR-PPAR-$\gamma$ & 0.75 & 0.97 & 0.61 & 0.99 & 0.23 & 0.96 & 0.23 & 0.31  \\
            SR-HSE & 0.75 & 0.94 & 0.61 & 0.99 & 0.23 & 0.94 & 0.23 & 0.32  \\
            NR-AR-LBD & 0.82 & 0.98 & 0.78 & 0.99 & 0.56 & 0.99 & 0.56 & 0.66  \\
            NR-ER & 0.69 & 0.88 & 0.64 & 0.96 & 0.32 & 0.89 & 0.32 & 0.40  \\
            SR-ARE & 0.78 & 0.86 & 0.67 & 0.95 & 0.39 & 0.88 & 0.39 & 0.47  \\
            SR-MMP & 0.87 & 0.89 & 0.75 & 0.96 & 0.54 & 0.93 & 0.54 & 0.62  \\
            NR-AhR & 0.85 & 0.91 & 0.73 & 0.96 & 0.50 & 0.93 & 0.50 & 0.55  \\
            NR-ER-LBD & 0.78 & 0.96 & 0.69 & 0.99 & 0.38 & 0.97 & 0.38 & 0.48  \\
            SR-ATAD5 & 0.75 & 0.96 & 0.61 & 0.99 & 0.22 & 0.97 & 0.22 & 0.32  \\
            SR-p53 & 0.79 & 0.94 & 0.64 & 0.99 & 0.29 & 0.96 & 0.29 & 0.40 \\
            CT-TOX & 0.79 & 0.92 & 0.61 & 0.97 & 0.25 & 0.84 & 0.25 & 0.31 \\[1pt]
            \hdashline
            \rule{0pt}{0.8\normalbaselineskip}  % <- create a tiny gap
            Average	& 0.78 & 0.93 & \textbf{0.67} & 0.98 & \textbf{0.36} & 0.94 & \textbf{0.36} & \textbf{0.45} \\
            \bottomrule
        \end{tabular}
    }
    \end{center}
    % \vspace{-0.2in}
\end{table}

==> tbl_tox_RF.tex <==
\begin{table}[!h]
    \begin{center}
    \caption{
        Performance on toxicity prediction for Random Forest on all 12 Tox21 tasks and ClinTox task (CT-TOX). The reported metrics are ROC AUC, accuracy, balanced accuracy, true negative rate, true positive rate, precision, recall, and the F1 score.
    }%
    \label{tbl:tox_RF} 
    \scalebox{0.85}{
        \begin{tabular}{r|
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        S[table-format=1.2]
        }
            \toprule
            {Task}
            & {AUC}
            & {ACC}
            & {BAC}
            & {TN}
            & {TP}
            & {PR}
            & {RC}
            & {F1}
            \\
            \midrule 
            % \underline{Train} & & & & \\[0.5mm]
            NR-AR & 0.78 & 0.98 & 0.73 & 0.99 & 0.46 & 0.99 & 0.46 & 0.60 \\
            NR-Aromatase & 0.81 & 0.96 & 0.60 & 0.99 & 0.21 & 0.98 & 0.21 & 0.32 \\
            NR-PPAR-gamma & 0.82 & 0.97 & 0.56 & 0.99 & 0.12 & 0.99 & 0.12 & 0.20 \\
            SR-HSE & 0.77 & 0.95 & 0.56 & 0.99 & 0.13 & 0.97 & 0.13 & 0.22 \\
            NR-AR-LBD & 0.85 & 0.98 & 0.77 & 0.99 & 0.54 & 0.99 & 0.54 & 0.66 \\
            NR-ER & 0.72 & 0.89 & 0.60 & 0.98 & 0.21 & 0.93 & 0.21 & 0.32 \\
            SR-ARE & 0.81 & 0.86 & 0.61 & 0.99 & 0.24 & 0.94 & 0.24 & 0.36 \\
            SR-MMP & 0.88 & 0.89 & 0.67 & 0.98 & 0.36 & 0.95 & 0.36 & 0.49 \\
            NR-AhR & 0.89 & 0.91 & 0.65 & 0.99 & 0.32 & 0.96 & 0.32 & 0.45 \\
            NR-ER-LBD & 0.80 & 0.96 & 0.65 & 0.99 & 0.31 & 0.99 & 0.31 & 0.45 \\
            SR-ATAD5 & 0.84 & 0.96 & 0.55 & 0.99 & 0.10 & 0.97 & 0.10 & 0.18 \\
            SR-p53 & 0.83 & 0.95 & 0.56 & 0.99 & 0.13 & 0.99 & 0.13 & 0.22 \\
            CT-TOX & 0.76 & 0.92 & 0.55 & 0.98 & 0.13 & 0.85 & 0.13 & 0.19 \\[1pt]
            \hdashline
            \rule{0pt}{0.8\normalbaselineskip}  % <- create a tiny gap
            Average & \textbf{0.81} & 0.94 & 0.62 & 0.99 & 0.25 & 0.96 & 0.25 & 0.36 \\
            \bottomrule
        \end{tabular}
    }
    \end{center}
    % \vspace{-0.2in}
\end{table}
